Approximate message passing from random initialization with applications to $\mathbb{Z}_{2}$ synchronization

This paper is concerned with the problem of reconstructing an unknown rank-one matrix with prior structural information from noisy observations. While computing the Bayes-optimal estimator seems intractable in general due to its nonconvex nature, Approximate Message Passing (AMP) emerges as an efficient first-order method to approximate the Bayes-optimal estimator. However, the theoretical underpinnings of AMP remain largely unavailable when it starts from random initialization, a scheme of critical practical utility. Focusing on a prototypical model called $\mathbb{Z}_{2}$ synchronization, we characterize the finite-sample dynamics of AMP from random initialization, uncovering its rapid global convergence. Our theory provides the first non-asymptotic characterization of AMP in this model without requiring either an informative initialization (e.g., spectral initialization) or sample splitting.

==> recursion.tex <==
\subsection{Proof of Lemma~\ref{lem:recursion}}
We will prove the lemma with induction. Notice that with random initialization, we have $\xi_0 = 0$ and $\Delta_{\alpha,0}=0$. As a result, the bound~\eqref{eq:xi-delta-1} holds for $t=0$. We will then show that as bound~\eqref{eq:xi-delta-1} holds for $t-1$, we can establish the bound~\eqref{eq:kappa-1} and bound~\eqref{eq:xi-delta-1} for $t$ and equation~\eqref{eq:eta_derivative_small} for $t$ when $\alpha_t\lesssim\sqrt{\lambda-1}n^{-0.1}$.
\subsubsection{Case I: $\alpha_t\lesssim\sqrt{\lambda-1}n^{-0.1}$}
\paragraph{Bound for derivatives of $\eta_t$ for small $x$.}
First, according to bound~\eqref{eq:xi-delta-1}, if $t\leq\frac{\log n}{\lambda-1}$ and $\alpha_t\lesssim \sqrt{\lambda-1}n^{-0.1}$, we have
\begin{align*}
\Vert\xi_{t-1}\Vert_2\lesssim\sqrt{\frac{t^3\log n}{n}}\lesssim \sqrt{\frac{\log^4 n}{n(\lambda-1)^3}}.
\end{align*}
Therefore, relation~\eqref{eqn:pi_t} in Lemma~\ref{lem:parameters} implies that
\begin{align*}
\lt(\ltwo{\xi_{t-1}}+\sqrt{\frac{t\log n}{n}}\rt)^{1/2}\lesssim \sqrt{\lambda-1}n^{-0.1},
\end{align*}
which directly leads to the result
\begin{align}
\pi_t &\lesssim \sqrt{\lambda-1}n^{0.4}.
\end{align}
Based on relation~\eqref{eqn:gamma_t_final} of Lemma~\ref{lem:parameters}, we have
\begin{align*}
(\gamma_t\pi_t)^{-2} = \alpha_t^2 + 1 + O\bigg(\frac{\pi_t^2}{n} + \Vert \xi_{t-1}\Vert_2 + \sqrt{\frac{t\log n}{n}}\bigg) = 1 + O\lt((\lambda-1)n^{-0.2}\log n\rt),
\end{align*}
which indicates that $\gamma_t\pi_t=1+O((\lambda-1)n^{-0.2}\log n)$. Therefore, by noticing that $|1-\tanh^2(x)|\leq 1$, we obtain that as $|x|\lesssim\sqrt{\frac{\log n}{n}}$,
\begin{align*}
\eta_t'(x) &= \gamma_t\pi_t(1-\tanh^2(\pi_t x)) = (1+O((\lambda-1)n^{-0.2})) \cdot \left(1+O(|\pi_t x|^2)\right)\\
&= 1+O((\lambda-1)n^{-0.2}\log n),\\
|\eta_t''(x)| &\lesssim  \pi_t\cdot |\pi_t x|\lesssim (\lambda-1)n^{0.8}|x|.
\end{align*}

\paragraph{Bound for $\kappa_t$.}
Recall the definition of $\kappa_{t}$ as 
\begin{align*}
\kappa_t^2 \defn \max\bigg\{\bigg\langle\int\left[ x\eta_t^{\prime}\left(\alpha_tv^\star+\frac{1}{\sqrt{n}}x\right)-\frac{1}{\sqrt{n}}\eta_t^{\prime\prime}\left(\alpha_tv^{\star}+\frac{1}{\sqrt{n}}x\right)\right]^2\varphi_n(\dx)\bigg\rangle, \\
\qquad\qquad\bigg\langle\int\left[\eta_t^{\prime}\left(\alpha_tv^\star+\frac{1}{\sqrt{n}}x\right)\right]^2\varphi_n(\dx)\bigg\rangle\bigg\}.
\end{align*}
Here, $\varphi_n(\cdot)$ denotes the density function for $\mathcal{N}\left(0,I_n\right)$ and $\langle x\rangle=\frac{1}{n}\sum_{i=1}^{n}x_i$. 

Before providing a control of $\kappa_{t}$, let us introduce some simplifications of these terms.  
First as each entry $\vstar_i \stackrel{\mathrm{i.i.d.}}{\sim}\mathsf{Unif}\{\frac{1}{\sqrt{n}}, -\frac{1}{\sqrt{n}}\}$, one can easily write 
\begin{align*}
&\bigg\langle\int\left[ x\eta_t^{\prime}\left(\alpha_tv^\star+\frac{1}{\sqrt{n}}x\right)-\frac{1}{\sqrt{n}}\eta_t^{\prime\prime}\left(\alpha_tv^{\star}+\frac{1}{\sqrt{n}}x\right)\right]^2\varphi_n(\dx)\bigg\rangle\\
&=\int\left[ x\eta_t^{\prime}\left(\alpha_tv^\star_1+\frac{1}{\sqrt{n}}x\right)-\frac{1}{\sqrt{n}}\eta_t^{\prime\prime}\left(\alpha_tv^{\star}_1+\frac{1}{\sqrt{n}}x\right)\right]^2\varphi(\dx)\\
&=\int\left[ x\eta_t^{\prime}\left(\frac{1}{\sqrt{n}}(\alpha_t+x)\right)-\frac{1}{\sqrt{n}}\eta_t^{\prime\prime}\left(\frac{1}{\sqrt{n}}(\alpha_t+x)\right)\right]^2\varphi(\dx),
\end{align*}
where $\varphi(\cdot)$ corresponds to the density function for $\mathcal{N}\left(0,1\right)$ and we use the fact that $\eta_t(\cdot)$ is symmetry around $0$ and the integration is over distribution $\mathcal{N}(0, I_n)$. Similarly, we obtain 
\begin{align*}
\bigg\langle\int\left[\eta_t^{\prime}\left(\alpha_tv^\star+\frac{1}{\sqrt{n}}x\right)\right]^2\varphi_n(\dx)\bigg\rangle=\int\left[\eta_{t}^{\prime}\Big(\frac{1}{\sqrt{n}}(\alpha_t + x)\Big)\right]^2\varphi(\dx).
\end{align*}
Therefore, it holds that
\begin{align*}
\kappa_t^2 = 
\max\bigg\{\int |I_1(x)|^2\varphi(\dx), ~
\int |I_2(x)|^2\varphi(\dx)\bigg\},
\end{align*}
where we denote
\begin{align*}
I_1(x) &\defn x\eta_{t}^{\prime}\Big(\frac{1}{\sqrt{n}}(\alpha_t + x)\Big)  - \frac{1}{\sqrt{n}}\eta_{t}^{\second}\Big(\frac{1}{\sqrt{n}}(\alpha_t + x)\Big),\\
%
I_2(x) &\defn\eta_{t}^{\prime}\Big(\frac{1}{\sqrt{n}}(\alpha_t + x)\Big).
\end{align*}
%It is sufficient to show that for some constant $c > 0$
%\begin{align} \label{eq:kappa-bound}
%\kappa_t \le 
%\left\{ \begin{array}{rcl}
%         1 + O\lt(n^{-0.2}t\log^3 n\rt)  & \mbox{for} & \alpha_t \lesssim n^{-0.1} \\
%         1 - c\alpha_t^2 + O\lt(\sqrt{\frac{t\log^4 n}{n\alpha_t^4}}\rt) & \mbox{for} & \alpha_t \gtrsim n^{-0.1}
  %              \end{array}\right.
%\end{align}
With these notations in mind, we denote denote the event $\mathcal{A} \defn \left\{x: \vert x\vert\leq\sqrt{12\log n}\right\}$. 
For $x\sim\mathcal{N}\left(0,1\right)$, it can be easily verified that $P(\mathcal{A})=1-O(n^{-12})$. 
% Then, we define the event $\mathcal{A}=\left\{x: \vert x\vert\leq\sqrt{12\log n}\right\}$. It can be observed that as $x\sim\mathcal{N}\left(0,\frac{1}{n}\right)$, we have $P(\mathcal{A})=1-O(n^{-12})$. We also note that as $|x|\leq\sqrt{12\log n}$ and that $v^{\star}=\frac{1}{\sqrt{n}}\text{ or }-\frac{1}{\sqrt{n}}$, we have
% \begin{align*}
% \left\vert\alpha_t v^\star + \frac{1}{\sqrt{n}}x\right\vert\lesssim\sqrt{\frac{\log n}{n}}.
% \end{align*}
Conditional on event $\mathcal{A}$ and when $\alpha_t \lesssim \sqrt{\lambda^2-1}n^{-0.1}$, one has 
\begin{align*}
\Big\vert \frac{1}{\sqrt{n}}(\alpha_t + x)\Big\vert\lesssim\sqrt{\frac{\log n}{n}}.
\end{align*}
Meanwhile, we note that $\sqrt{\lambda+1}\asymp 1$, therefore $\alpha_t\lesssim \sqrt{\lambda^2-1}n^{-0.1}$ is equivalent to $\alpha_t\lesssim \sqrt{\lambda-1}n^{-0.1}$. As a result, according to equation~\eqref{eq:eta_derivative_small} established in the previous paragraph, when $|z| \lesssim \sqrt{\frac{\log n}{n}}$, it holds true that  
\begin{align}
\eta_t^{\prime}(z)= 1+ O((\lambda-1)n^{-0.2}\log n),\qquad |\eta_t''(z)|\lesssim (\lambda-1)n^{0.8} |z|.
\end{align}
Hence, in this case, we bound the difference between $I_1(x)$ and $x$ uniformly as 
\begin{align}
|I_1(x)-x|
&\notag\leq\lt|\eta_{t}^{\prime}\Big(\alpha_tv^{\star} + \frac{1}{\sqrt{n}}x\Big)-1\rt||x| + \frac{1}{\sqrt{n}}\lt|\eta_{t}^{\second}\Big(\alpha_tv^{\star} + \frac{1}{\sqrt{n}}x\Big)\rt|\\
%
&\notag=O\lt((\lambda-1)n^{-0.2}\log n\rt)+O((\lambda-1)n^{0.3})\lt|\alpha_t v^{\star}+\frac{1}{\sqrt{n}}x\rt|\\
&\notag\lesssim O\lt((\lambda-1)n^{-0.2}\log n\rt)+O\lt((\lambda-1)n^{0.3}\rt)\lt(\frac{1}{\sqrt{n}}+\frac{1}{\sqrt{n}}|x|\rt)\\
&=O\lt((\lambda-1)n^{-0.2}\log n\rt)(1+|x|).
\end{align}

In addition, for any $x\in\mathbb{R}$, based on Lemma~\ref{lem:eta_property} --- which suggests $|\eta_t'(x)|\lesssim 1$, $|\eta_t''(x)|\lesssim \sqrt{n}$ --- we observe that $|I_1(x)|\lesssim |x|+1$. 
As a result, it holds that
\begin{align}
\label{eqn:I-1}
\notag &\int |I_1(x)|^2\varphi(\dx) \\
%
\notag&= \int x^2\varphi(\dx) + \int (I_1(x)-x)(I_1(x)+x) \varphi(\dx)  \\
\notag&= 1 + \int_{\mathcal{A}} (I_1(x)-x)(I_1(x)+x) \varphi(\dx) + \int_{\mathcal{A}^{\mathsf{c}}} (I_1(x)-x)(I_1(x)+x) \varphi(\dx) \\
\notag&= 1 + O\lt(\int_\mathcal{A} (\lambda-1)n^{-0.2}\log n\cdot (|x|+1)^2\varphi(\dx) + \int_{\mathcal{A}^c} (|x|+1)^2\varphi(\dx)\rt) \\
%
&= 1 + O\lt((\lambda-1)n^{-0.2}\log n\rt),
\end{align}
where the last equality utilizes the fact that for $c_n=\sqrt{12\log n}$,
\begin{align*}
\int_{\mathcal{A}^c}x^2\varphi(\dx)
= 2 \int_{c_n}^{\infty} x^2\varphi(\dx) \lesssim \int_{c_n}^{\infty} x^2 \exp\lt(-\frac{1}{2}x^2\rt)\dx 
%
&\lesssim \int_{c_n^2}^{\infty} \sqrt{x} \exp\lt(-\frac{1}{2}x\rt) \dx \\
%
&\lesssim c_n^2\exp \lt(-\frac{1}{2}c_n^2\rt) \lesssim \frac{\log n}{n^6}.
\end{align*} 
%
Regarding the term $I_2(x)$, equation~\eqref{eq:eta_derivative} of Lemma~\ref{lem:eta_property} implies that $|I_2(x)|\lesssim 1$. 
Furthermore, if $|x|\leq\sqrt{12\log n}$, based on equation~\eqref{eq:eta_derivative_small} established in the previous paragraph, we have $|I_2(x)| = 1+ O((\lambda-1)n^{-0.2}\log n)$. Putting these together, we obtain that
\begin{align}\begin{aligned}\label{eqn:I-2}
\int |I_2(x)|^2\varphi(\dx) &= \int_\mathcal{A} |I_2(x)|^2\varphi(\dx) +\int_{\mathcal{A}^c} |I_2(x)|^2\varphi(\dx) \\ 
&= 1+ O((\lambda-1)n^{-0.2}\log n + P(\mathcal{A}^c)) \\
&= 1+ O((\lambda-1)n^{-0.2}\log n).
\end{aligned}\end{align}
Combining inequalities \eqref{eqn:I-1} and~\eqref{eqn:I-2} leads to 
\begin{align*}
\kappa_t^2 = 1 + O\lt((\lambda-1)n^{-0.2}\log n\rt)= 1+o\lt(\frac{\lambda-1}{\log n}\rt).
\end{align*}

\paragraph{Bound for $\xi_t$ and $\Delta_{\alpha,t}$.}
As we have established the bound of $\kappa_t$, substituting property \eqref{eq:kappa-1} into \eqref{eqn:christmas} yields 
\begin{align}
\label{eqn:merry}
\|\xi_{t}\|_{2} 
% &\le \sqrt{\kappa_t + \sqrt{\frac{t\log^2 n}{n}}} \|\xi_{t-1}\|_{2}+O\Bigg(\sqrt{\frac{t\log n}{n}} +\sqrt{t\log n}\|\xi_{t-1}\|_{2}^{2}+\sqrt{\frac{{t\log n}}{n}}\|\xi_{t-1}\|_{2}\Bigg) \notag\\
%
&\le \sqrt{ 1+ o\left(\frac{\lambda-1}{\log n}\right)+\sqrt{\frac{t\log^2 n}{n}} } \|\xi_{t-1}\|_{2}+O\Bigg(\sqrt{\frac{t\log n}{n}} +\sqrt{t\log n}\|\xi_{t-1}\|_{2}^{2}+\sqrt{\frac{{t\log n}}{n}}\|\xi_{t-1}\|_{2}\Bigg) \notag\\
&\le \bigg(1 + o\left(\frac{\lambda-1}{\log n}\right)\bigg) \|\xi_{t-1}\|_{2}+O\bigg(\sqrt{\frac{t\log n}{n}}\bigg).
\end{align}
Here in the last line, we remind the readers $t \leq \frac{C\log n}{\lambda - 1}$ and $\lambda - 1\gtrsim n^{-1/9}.$
In addition, invoking the inductive assumption $\|\xi_{t}\|_2 \lesssim \sqrt{\frac{(t-1)^3\log n}{n}}$ gives 
\begin{align*}
	\sqrt{t\log n}\|\xi_{t-1}\|_{2}+\sqrt{\frac{{t\log n}}{n}} = o\left(\frac{\lambda-1}{\log n}\right). 
\end{align*}
%\yutingcomment{why? add details}
Invoking the relation~\eqref{eqn:merry} recursively gives the bound for $\ltwo{\xi_t}$ as
\begin{align*}
\|\xi_{t}\|_{2} 
&\le \bigg(1 + o\bigg(\frac{\lambda-1}{\log n}\bigg)\bigg)^{t-1} \|\xi_1\|_{2} + 
O\Bigg( \sum_{j=2}^{t} \bigg(1 + o\big(\frac{\lambda-1}{\log n}\big)\bigg)^{t-j} \sqrt{\frac{j\log n}{n}}\Bigg)\\
&\lesssim \ltwo{\xi_1} + O\Bigg( \sum_{j=2}^{t} \bigg(1 + o\big(\frac{\lambda-1}{\log n}\big)\bigg)^{t-j}\Bigg)\cdot\sqrt{\frac{t\log n}{n}}\\
&\lesssim \sqrt{\frac{t\log n}{n}},
\end{align*}
where we utilize the fact that $t \lesssim \frac{\log n}{\lambda - 1}$. Furthermore, combining equation~\eqref{eqn:delta-alpha-general} and equation~\eqref{eqn:ABD} with bound of $\ltwo{\xi_t}$, we easily establish the bound for $\Delta_{\alpha,t}$ and validatates equation~\eqref{eq:xi-delta-1}.

\subsubsection{Case II: $\sqrt{\lambda-1}n^{-0.1}\lesssim \alpha_t\lesssim \sqrt{\lambda^2-1}$}
In this case, we only show the proof for $\kappa_t$, while the proof of bound for $\ltwo{\xi_t}$ and $\Delta_{\alpha,t}$ follows the same way as we did in Case I.
\paragraph{Bound for $\kappa_t$}

%Notice that when $\alpha_t \ge \sqrt{\lambda^2 - 1}$, a satisfactory bound is already given in~\citet[Section D.3.4]{li2022non}, where it is shown therein that 
%\begin{align}
%  \kappa_t^2 \leq 1 - \frac{1}{15}(\lambda - 1).
%\end{align}

%In the remaining case, we first claim that the following properties regarding $\pi_t$ and $\gamma_t$ hold true
Here, we note that as bound~\eqref{eq:xi-delta-1} holds for $t-1$, based on equation~\eqref{eqn:pi_t} of Lemma~\ref{lem:parameters}, we have
\begin{align}\label{equ:pi-alpha}
\pi_t &= \sqrt{n}\alpha_t+\frac{\sqrt{n}}{\alpha_t}O\bigg(\Vert\xi_{t-1}\Vert_2+\sqrt{\frac{t\log n}{n}}\bigg)=\alpha_t\sqrt{n} + \sqrt{n}O\lt(\sqrt{\frac{(t + \log^3 n/(\lambda-1))\log n}{n(\lambda-1)^2\alpha_t^2}}\rt).
\end{align}
We also note that as $\alpha_t\gtrsim\sqrt{\lambda^2-1}n^{-0.1}$, we have $\pi_t\lesssim\sqrt{n}\alpha_t$.
\yutingcomment{why? what is the assumption on $t$?} Therefore, based on equation~\eqref{eqn:gamma_t} of Lemma~\ref{lem:parameters}, we have
\begin{align}
\gamma_t^{-2} &=n\int \tanh^2\lt(\frac{\pi_t}{\sqrt{n}}(\alpha_t + x)\rt)\varphi(\dx) + \pi_t^2O\bigg(\Vert \xi_{t-1}\Vert_2 + \sqrt{\frac{t\log n}{n}}\bigg)\notag\\
&=n\int \tanh^2\lt(\frac{\pi_t}{\sqrt{n}}(\alpha_t + x)\rt)\varphi(\dx) + \alpha_t^2O\bigg(\sqrt{\frac{n(t + \log^3 n/(\lambda-1))\log n}{(\lambda-1)^2}}\bigg). 
%\label{eq:pi-gamma}
\end{align}
%Let us take these properties as given for the moment, and come back to their proofs at the end of this section. 
In view of the definition of $\eta_{t}(\cdot),$ we record several basic facts as follows 
\begin{gather}
\begin{aligned}
\label{eqn:super-basic}
  \eta_{t}^{\prime}(x) &= \gamma_t\pi_t\big(1-\tanh^2(\pi_tx)\big) \\
  \eta_{t}^{\second}(x) &= -2\gamma_t\pi_t^2\tanh(\pi_tx)\big(1-\tanh^2(\pi_tx)\big)\\ 
  \eta_{t}^{(\third)}(x) &= -2\gamma_t\pi_t^3\big(1-\tanh^2(\pi_tx)\big)\big(1-3\tanh^2(\pi_tx)\big),
\end{aligned}
\end{gather}
and hence, 
\begin{align}
\label{eqn:I1-allegro}
\int |I_1(x)|^2\varphi(\dx) 
%& =  \int\Bigg[x\eta_{t}^{\prime}\Big(\alpha_{t}v^{\star}+\frac{1}{\sqrt{n}}x\Big)-\frac{1}{\sqrt{n}}\eta_{t}^{\second}\Big(\alpha_{t}v^{\star}+\frac{1}{\sqrt{n}}x\Big)\Bigg]^{2}\varphi_{n}(\dx)\\
%
 & =\int\lt[\lt(\gamma_{t}\pi_{t}x+\frac{2}{\sqrt{n}}\gamma_{t}\pi_{t}^{2}\tanh\Big(\frac{\pi_{t}}{\sqrt{n}}\big(\alpha_{t}+x\big)\Big)\rt)\cdot\Big(1-\tanh^{2}\Big(\frac{\pi_{t}}{\sqrt{n}}\big(\alpha_{t}+x\big)\Big)\Big)\rt]^{2}\varphi(\dx) \\
 %& = \int\lt[\lt(\mu_{t}\alpha_{t}x+2\mu_{t}\alpha_{t}^{2}\tanh\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\rt)\cdot\Big(1-\tanh^{2}\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\Big)\rt]^{2}\varphi(\dx) + O\lt(\sqrt{\frac{t\log^3 n}{n\alpha_t^4}}\rt), 
 %
 \label{eqn:I2-allegro}
\int |I_2(x)|^2\varphi(\dx) &= \int \Big[\gamma_t\pi_t\big(1-\tanh^{2}\Big(\frac{\pi_{t}}{\sqrt{n}}\big(\alpha_{t}+x\big)\Big)\Big)\Big]^2 \varphi(\dx).
\end{align}
The rest of this section is devoted to control the right hand sides of the above two expressions with 
$\sqrt{\lambda^2-1}n^{-0.1}\lesssim \alpha_t \le \sqrt{\lambda^2-1}.$

For notational convenience, let us introduce the following shorthand expressions  
\begin{align*}
J_1(x) &\defn \gamma_{t}\pi_{t}x+\frac{2}{\sqrt{n}}\gamma_{t}\pi_{t}^{2}\tanh\Big(\frac{\pi_{t}}{\sqrt{n}}\big(\alpha_{t}+x\big)\Big), \\
J_2(x) &\defn \mu_{t}\alpha_{t}x+2\mu_{t}\alpha_{t}^{2}\tanh\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big),\\
K_1(x)   &\defn 1-\tanh^{2}\Big(\frac{\pi_{t}}{\sqrt{n}}\big(\alpha_{t}+x\big)\Big),\\
K_2(x)   &\defn 1-\tanh^{2}\Big(\alpha_t\big(\alpha_{t}+x\big)\Big).
\end{align*}
With these notation in place, following \eqref{eqn:I1-allegro}, we shall write 
\begin{align}
\notag \int |I_1(x)|^2\varphi(\dx) 
&= \int [J_1(x)K_1(x)]^2\varphi(\dx) \\
%
\notag &= \int [J_2(x)K_2(x)]^2\varphi(\dx) +O\lt(\int \lt\vert J_2(x)\rt\vert^2\lt\vert K_1(x)-K_2(x)\rt\vert\lt\vert K_1(x)+K_2(x)\rt\vert\varphi(\dx)\rt)\\
%
&\qquad\qquad+O\lt(\int\vert J_1(x)-J_2(x)\vert\vert J_1(x)+J_2(x)\vert\vert K_1(x)\vert^2\varphi(\dx)\rt).
%
% &= \int [J_2(x)K_2(x)]^2\varphi(\dx) +   O\lt(\frac{1}{\alpha_t}\sqrt{\frac{t\log^3 n}{n}}\rt)\int(|x|+\alpha_t)^3\varphi(\dx). 
\label{eqn:I1-adagio}
\end{align}
To bound $\int |I_1(x)|^2\varphi(\dx)$, it is thus sufficient to control these three terms on the right respectively. 
Before proceeding, we find it helpful to make note of several preliminary properties. 
First, if we denote 
\begin{align*}
\mu_{t} \defn \lt[\int\tanh^{2}\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\varphi(\dx)\rt]^{-\frac{1}{2}},
\end{align*}
one can verify that
\begin{align}
\label{eqn:ut-num}
  \mu_t\asymp \alpha_t^{-1}.
\end{align}
In order to see this, the fact that $\tanh^2(x) \leq x^{2}$ implies that 
\begin{align*}
  \int\tanh^2(\alpha_t(\alpha_t+x))\varphi(\dx)\leq \int\alpha_t^2(\alpha_t+x)^2\varphi(\dx)\lesssim \alpha_t^2, \qquad \text{for } \alpha_t \leq \lambda.
\end{align*}
On the other hand, when $|x| \leq 1/2$, $\alpha_{t}\in (0,\lambda]$ and $\lambda \in (1,1.2]$,  $\alpha_t(\alpha_t+x) \subset [-0.0625, 2.04]$ where $\tanh^2(x)/x^2 \geq  0.22$. 
\begin{align*}
\int\tanh^2(\alpha_t(\alpha_t+x))\varphi(\dx)&\geq \int\tanh^2(\alpha_t(\alpha_t+x))\textbf{1}(\vert x\vert\leq 0.5)\varphi(\dx)\\
&\gtrsim\int\alpha_t^2(\alpha_t+x)^2\textbf{1}(\vert x\vert\leq 0.5)\varphi(\dx)
\gtrsim \alpha_t^2.
\end{align*}
Additionally, by definition, it obeys that 
\begin{align}\label{equ:gamma-mu}
\gamma_t &=\lt[ n\mu_t^{-2} +O\lt(\sqrt{n(t + \log^3 n/(\lambda-1))\log n}\rt)\rt]^{-1/2} \notag\\
&= \frac{\mu_t}{\sqrt{n}}\lt(1+O\lt(\frac{\mu_t^2}{n}\sqrt{n(t + \log^3 n/(\lambda-1))\log n}\rt)\rt)\asymp\frac{\mu_t}{\sqrt{n}}.
\end{align}
%and
%\begin{align}
%\mu_t = \sqrt{n}\gamma_t \lt(1+O\lt(\frac{1}{n\gamma_t^2}\sqrt{\frac{t\log^3 n}{n}}\rt)\rt).
%\end{align}
Based on~\eqref{equ:pi-alpha} and~\eqref{equ:gamma-mu}, some direct algebra further leads to 
\begin{align}
\lt\vert\gamma_t\pi_t-\mu_t\alpha_t\rt\vert &\lesssim \mu_t\alpha_t\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\left(\frac{1}{\alpha_t^2(\lambda-1)}+\mu_t^2\right)\notag\\
\label{equ: bound-kappa-t-1}
&\lesssim \frac{1}{\alpha_t^2(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}},\\
\label{equ: bound-kappa-t-2}
\lt\vert\frac{1}{\sqrt{n}}\gamma_t\pi_t^2-\mu_t\alpha_t^2\rt\vert &\lesssim \mu_t\alpha_t^2\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\left(\frac{1}{\alpha_t^2(\lambda-1)}+\mu_t^2\right)\notag \\
&\lesssim \frac{1}{\alpha_t(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}},\\
\label{equ: bound-kappa-t-3}
\lt\vert\frac{\pi_t}{\sqrt{n}}-\alpha_t\rt\vert & \lesssim \frac{1}{\alpha_t(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}. 
\end{align}
Taking inequalities~\eqref{equ: bound-kappa-t-1}-\eqref{equ: bound-kappa-t-3} collectively with the fact that $\mu_t\alpha_t^2\asymp \alpha_t$, we obtain
\begin{align}
\label{bound-K1-K2}
\lt\vert K_1(x) - K_2(x)\rt\vert \lesssim & \lt\vert\frac{\pi_t}{\sqrt{n}}-\alpha_t\rt\vert\lt\vert\alpha_t +x\rt\vert \lesssim \frac{1}{\alpha_t(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\cdot (\vert x\vert + \alpha_t),
\end{align}
and 
\begin{align}\label{bound-J1-J2}
\lt\vert J_1(x) - J_2(x)\rt\vert &\leq  \lt\vert\gamma_t\pi_t-\mu_t\alpha_t\rt\vert \vert x\vert + 2\lt\vert\frac{1}{\sqrt{n}}\gamma_t\pi_t^2-\mu_t\alpha_t^2\rt\vert\lt\vert\tanh\lt(\frac{\pi_t}{\sqrt{n}}(\alpha_t+x)\rt)\rt|\notag \\
&\qquad\qquad + \mu_t\alpha_t^2\lt\vert\tanh\lt(\frac{\pi_t}{\sqrt{n}}(\alpha_t+x)\rt) - \tanh\lt(\alpha_t(\alpha_t+x)\rt)\rt\vert \notag \\
&\lesssim \frac{1}{\alpha_t^2(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\vert x\vert +  \frac{1}{\alpha_t(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}} \notag\\
&\qquad\qquad + \frac{1}{(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}} (\vert x\vert+\alpha_t)\notag\\
&\lesssim  \frac{1}{\alpha_t^2(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}(\vert x\vert+\alpha_t).
\end{align}


Equipped the above relations, we are positioned to control the right hand side of expression~\eqref{eqn:I1-adagio}. 
Combining~\eqref{bound-K1-K2} and \eqref{bound-J1-J2} directly yields 
\begin{align}
\notag &\int |I_1(x)|^2\varphi(\dx)  \\
% &= \int [J_1(x)K_1(x)]^2\varphi(\dx) \\
% &= \int [J_2(x)K_2(x)]^2\varphi(\dx) +O\lt(\int \lt\vert J_2(x)\rt\vert^2\lt\vert K_1(x)-K_2(x)\rt\vert\lt\vert K_1(x)+K_2(x)\rt\vert\varphi(\dx)\rt)\\
% &\qquad\qquad+O\lt(\int\vert J_1(x)-J_2(x)\vert\vert J_1(x)+J_2(x)\vert\vert K_1(x)\vert^2\varphi(\dx)\rt) \\
\notag &= \int [J_2(x)K_2(x)]^2\varphi(\dx) + O\left( \frac{1}{\alpha_t(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\right)\cdot \int(\vert x\vert + \alpha_t)^3\varphi(\dx) \\
%
\notag&\qquad\qquad+ O\left(\frac{1}{\alpha_t^2(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\right)\cdot\int(\vert x\vert+\alpha_t)^2\varphi(\dx) \\
%
&=  \int \Big[\mu_{t}\alpha_{t}x+2\mu_{t}\alpha_{t}^{2}\tanh\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\Big]^2\Big[1-\tanh^{2}\Big(\alpha_t\big(\alpha_{t}+x\big)\Big)\Big]^2\varphi(\dx)\notag\\
&\qquad\qquad+O\left( \frac{1}{\alpha_t^2(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\right),
\label{eqn:I1-rondo}
\end{align}
where the first line invokes the simple observations that $\vert J_i(x)\vert\lesssim |x|+\alpha_t$ and $\vert K_i(x)\vert\lesssim 1$ for $i=1,2$.
Similarly, one can derive in the same manner that  
\begin{align}
\int|I_2(x)|^2\varphi(\dx)
&= \mu_{t}^2\alpha_{t}^2\int \lt[1-\tanh^2\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\rt]^2 \varphi(\dx) \notag\\
&\qquad+ O\left( \frac{1}{\alpha_t^2(\lambda-1)}\sqrt{\frac{(t+\log^3 n/(\lambda-1))\log n}{n}}\right). 
\end{align}
Hence to establish bound~\eqref{eq:kappa-1}, since
\begin{align*}
\kappa_t^2 = 
\max\bigg\{\int |I_1(x)|^2\varphi(\dx), ~
\int |I_2(x)|^2\varphi(\dx)\bigg\},
\end{align*}
we are only left to show that
\begin{subequations}
\label{eqn:I12-finale}
\begin{align}
\int \Big[\mu_{t}\alpha_{t}x+2\mu_{t}\alpha_{t}^{2}\tanh\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\Big]^2\Big[1-\tanh^{2}\Big(\alpha_t\big(\alpha_{t}+x\big)\Big)\Big]^2\varphi(\dx) &\le 1 - c\alpha_t^2; \\
\mu_{t}^2\alpha_{t}^2\int \lt[1-\tanh^2\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\rt]^2 \varphi(\dx) &\le 1 - c\alpha_t^2.
\end{align}
\end{subequations}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Proof of relation \eqref{eqn:I12-finale}.} 
To proceed, consider the task of recovering $\vstar$ with $\vstar_{i} \sim \mathsf{Unif}\{\pm\frac{1}{n}\}$ by observing $Y = \alpha_t \vstar + g$ for $g \sim \mathcal{N}(0,\frac{1}{n}I_n)$. As mentioned before, the Bayes optimal denoising function satisfies 
\begin{align*}
  \eta_t \propto \Exs[\vstar \,\mid\, Y] = \tanh(\alpha_t Y),
\end{align*}
where $\Exs[\vstar \,\mid\, Y]$ corresponds to the minimum mean square estimator (MMSE).
As a result, it satisfies that 
\begin{align}
  \operatorname{Cor}\lt(\vstar, f(Y)\rt)\leq\operatorname{Cor}\lt(\vstar, \Exs[\vstar\,\mid\,Y]\rt),
\end{align}
for any measurable function $f$. 
In particular, the Bayes optimal function outperforms the identity denosing function which means  
\begin{align}
  \notag \frac{\Exs \inprod{\vstar}{\alpha_t \vstar + g}}{\sqrt{\Exs \ltwo{\alpha_t \vstar + g}^2}}
   \leq 
   \frac{\Exs \inprod{\vstar}{\tanh(\alpha_t (\alpha_t \vstar + g))}}{\sqrt{\Exs \ltwo{\tanh(\alpha_t (\alpha_t \vstar + g)}^2}}
   &=
   \frac{\int \tanh(\alpha_t (\alpha_t + x)) \varphi(dx)}{\sqrt{\int \tanh^2(\alpha_t (\alpha_t + x)) \varphi(\dx)}} \\
%
   &=
   \sqrt{\int \tanh^2(\alpha_t(\alpha_t + x)) \varphi(\dx)},
\end{align}
where the fist equality holds due to the symmetry of $\vstar$ along with the symmetry of $\varphi(\cdot)$;
the second equality holds since $\int \tanh(\alpha^2 + \alpha x) \varphi(\dx) = \int \tanh^2(\alpha^2 + \alpha x) \varphi(\dx).$
As a consequence, the above relation suggests that 
\begin{align}
\label{eqn:bayes-opt}
\frac{\alpha_t}{\sqrt{\alpha^2_t + 1 }} = 
  \frac{\Exs \inprod{\vstar}{\alpha_t \vstar + g}}{\sqrt{\Exs \ltwo{\alpha_t \vstar + g}^2}} \leq \sqrt{\int \tanh^2(\alpha_t(\alpha_t + x)) \varphi(\dx)} = 
  \frac{1}{\mu_t},
\end{align}
which in turns suggests $\mu_t\alpha_t \le \sqrt{\alpha_t^2 + 1} = : \gamma$. 
%since 
%\begin{align*}
%\left(\frac{\lambda}{\mu_t}\right)^2 = \lambda^2 \int\tanh^{2}\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\Big)\varphi(\dx) > \alpha_t^2,
%\end{align*}
%which holds in the same way as the monotonicity of $\tau_t$ in~\citet{li2022non} (cf.~(254)). \yutingcomment{different range of $\alpha_t$?}
%In addition, \yutingcomment{add explanations}
Armed with this relation, we can conclude that 
\begin{align*}
&\max\bigg\{\int \Big[\mu_{t}\alpha_{t}x+2\mu_{t}\alpha_{t}^{2}\tanh\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\Big]\Big[1-\tanh^{2}\Big(\alpha_t\big(\alpha_{t}+x\big)\Big)\Big]\varphi(\dx), \\
&\qquad\qquad\qquad\qquad\mu_{t}^2\alpha_{t}^2\int \lt[1-\tanh^2\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\rt]^2 \varphi(\dx)\bigg\} \\
&\le \gamma^2\max\bigg\{\int \Big[x+2\alpha_{t}\tanh\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\Big]\Big[1-\tanh^{2}\Big(\alpha_t\big(\alpha_{t}+x\big)\Big)\Big]\varphi(\dx), \\
&\qquad\qquad\qquad\qquad\int \lt[1-\tanh^2\Big(\alpha_{t}\big(\alpha_{t}+x\big)\Big)\rt]^2 \varphi(\dx)\bigg\} \\
&=: \kappa^2(\gamma, \alpha_t^2).
\end{align*}
To bound the right hand side, since $\gamma \defn \sqrt{\alpha^2_{t}+1}$, relation~(272) in \cite{li2022non} indicates 
that 
\begin{align}
  \kappa^2(\gamma, \alpha_t^2) \le 1 - O(\gamma - 1) \le 1 - c\alpha_t^2.
\end{align}
Here, notice that we view $\gamma$ and $\alpha_t^2$ as $\lambda$ and $\tau$ in~(272) of~\citet{li2022non}, respectively. Putting everything together completes the proof of the required relation~\eqref{eqn:I12-finale}.
We thus complete the proof of Lemma~\ref{lem:recursion}. 
